Prompting and Fine-Tuning Open-Sourced Large Language Models for Stance Classification

Stance classification, the task of predicting the viewpoint of an author on a subject of interest, has long been a focal point of research in domains ranging from social science to machine learning. Current stance detection methods rely predominantly on manual annotation of sentences, followed by training a supervised machine learning model. However, this manual annotation process requires laborious annotation effort, and thus hampers its potential to generalize across different contexts. In this work, we investigate the use of Large Language Models (LLMs) as a stance detection methodology that can reduce or even eliminate the need for manual annotations. We investigate 10 open-source models and 7 prompting schemes, finding that LLMs are competitive with in-domain supervised models but are not necessarily consistent in their performance. We also fine-tuned the LLMs, but discovered that fine-tuning process does not necessarily lead to better performance. In general, we discover that LLMs do not routinely outperform their smaller supervised machine learning models, and thus call for stance detection to be a benchmark for which LLMs also optimize for. The code used in this study is available at \url{https://github.com/ijcruic/LLM-Stance-Labeling}

==> main_old_snippets.tex <==
Stance detection, the task of predicting an author's viewpoint towards a subject of interest, has long been a focal point of research. Current stance detection methods predominantly rely on manual annotation of sentences, followed by training a supervised machine learning model. This manual annotation process, however, imposes limitations on the model's ability to fully comprehend the stances in the sentence and hampers its potential to generalize across different contexts. In this study, we investigate the use of Large Language Models (LLMs) for the task of stance classification, with an absolute minimum use of human labels. We scrutinize four distinct types of prompting schemes combined with LLMs, comparing their accuracies with manual stance determination. Our study reveals that while LLMs can match or sometimes even exceed the benchmark results in each dataset, their overall accuracy is not definitively better than what can be produced by supervised models. This suggests potential areas for improvement in the stance classification for LLMs. The application of LLMs, however, opens up promising avenues for unsupervised stance detection, thereby curtailing the need for manual collection and annotation of stances. This not only streamlines the process but also paves the way for expanding stance detection capabilities across languages. Through this paper, we shed light on the stance classification abilities of LLMs, thereby contributing valuable insights that can guide future advancements in this domain. The code used in this study is made available at \url{https://github.com/ijcruic/LLM-Stance-Labeling}.

\subsection{Stance Classification Task}
Stance classification is a well-studied natural language processing task, with several benchmark datasets and shared tasks created. In previous work involving stance classification, much of the focus was on the construction of supervised machine-learning models for the task. A commonly used machine learning classifier is the Support Vector Machine \cite{lai2018stance,elfardy2016cu}, which has performed well in the SemEval-2016 stance detection competition \cite{mohammad2016semeval}. Supervised models that use neural network architectures are also popular. These include the use of convolutional neural networks \cite{wei2016pkudblab}, or recurrent neural networks \cite{zarrella2016mitre}, sometimes enhanced with textual entailment \cite{zhao2020pretrained} and data augmentation for improved accuracies \cite{kawintiranon2021knowledge}. Most recent work, however, has focused on multi-task learning objectives and transfer learning from transformer-based neural networks \cite{alturayeif2023systematic, yang-etal-2019-blcu, zhao2020pretrained}. Despite the typically stronger in-domain performance of these models, they often struggle to generalize to new data or other targets of stances, and are often of little use to real-world practitioners due to these generalizability shortcomings \cite{ng2022my,alturayeif2023systematic}.

While most work in stance classification has focused on supervised machine learning techniques, there are also some unsupervised techniques. Unsupervised learning methods make use of the idea of language homogenity for label classification \cite{zhang2023doubleh}. In that aspect, graph networks are a popular technique. \citet{zhang2023doubleh} used graph neural networks to formulate homogeneous and heterogenous information for a user on Twitter, inferring the stance based on past tweets and tweets of neighbors. Another technique is label propagation based on the user interaction network or relationships \cite{10.1145/2492517.2492557}, to propagate stance labels based on existing knowledge. The interaction network can also be divided into partitions, with the stance of each partition then interpreted \cite{pick2022stem}. \citet{darwish2020unsupervised} first projected a large set of Twitter user data to a low-dimensional space before clustering the interaction network into multiple partitions. While these methods do not rely on having a set of stance labels to train a model, they often rely on very specific scenarios for their use (i.e., a social media website that has explicit behavioral links between users, which can be used to create a network) and strong assumptions about the language or behavior of users to infer stance (i.e., use of a certain word or hashtag always conveys a certain stance).

Recently, there has been an increase in research focusing on the concept of zero-shot stance detection. Notably, \cite{allaway2023zero} discuss a variety of techniques for zero-shot stance detection and present an adaptation of the SemEval2016 dataset \cite{zarrella2016mitre}, along with their own VAST dataset, specifically designed for this purpose. They highlight the multitude of ways stance characterization can be achieved in a zero-shot manner. According to \cite{allaway2023zero}, there are three primary paradigms of zero-shot stance detection: topic, language, and genre. For each paradigm, a model is typically trained on all data, except for one element of the paradigm which is reserved for the zero-shot test. For instance, in zero-shot topic stance detection, a model is trained on data from all topics except one, which is then used for evaluation. \cite{allaway2023zero} found that all models perform less optimally in the zero-shot setting compared to a fully supervised setting.

\subsection{The use of Large Language Models for Stance Classification}
Large Language Models (LLMs) have the capability to process and evaluate sentences of natural languages. These models have been used for tasks ranging from reading comprehension to mathematical problem solving \cite{zheng2023judging}. These models are trained on an enormous amount of data and have an uncanny ability to evaluate sentences and respond to input prompts, thus it is not surprising that researchers investigate using these models for the stance detection task. \autoref{tab:stance_llm} lists a table of current works involving stance detection using LLMs.

While there is a suite of LLMs invented, much of current work has focused on solely ChatGPT, producing mixed results. \cite{zhang2022would} found that with just an instruction-based prompt (although they hint at the use of reasoning in a prompt in their paper), ChatGPT could produce better results on the SemEval2016 benchmark data set than supervised models. However, \citet{aiyappa2023can} examined the stance detection task using the ChatGPT model, observing that while there is a boost in performance, there could be potential contamination of data through its massive trained dataset, therefore making the evaluation unreliable. Additionally, \citet{mets2023automated} probed the usability of ChatGPT as a zero-shot classifier, using only a task-based prompt, for stance detection on a custom data set on the topic of immigration in various language news articles. They found that ChatGPT performed close to the best supervised model, but was ultimately inferior for the stance classification task. Finally, given the similarities between stance and sentiment, it is also worth mentioning that \cite{kheiri2023sentimentgpt} investigated all of the OpenAI model offerings on the task of sentiment classification with a couple of different prompts and different benchmark data sets and found that GPT models, especially if fine-tuned, can significantly outperform any other models for sentiment classification. Overall, it is still unclear if LLMs, especially with prompt engineering and without the use of fine-tuning on labeled data, can perform the task of stance classification.

With the advent of LLMs for natural language tasks, the new discipline of prompt engineering has also come into being. Prompt engineering is the discipline of finding the right ways to provide input to models --- or `prompt' them --- to get the best outputs \cite{schmidtcataloging, white2023prompt, Ramlochan2023prompt}. While this is a fast-changing discipline, with new findings about prompt engineering constantly emerging, there are a couple of techniques that have emerged for use with LLMs in particular. The first is few-shot prompting, which is when you give a few examples of what you want the LLM to do as part of the prompt \cite{white2023prompt, brown2020language, wei2023larger}. This is different from fine-tuning the LLM or low-shot learning, as no training (i.e., adjusting of model weights) is performed when the examples are given; the examples are only given as part of the context of the task \cite{brown2020language}. While this prompting technique does consistently produce improved outputs, there are still possible instabilities in the technique which can be caused by things like the ordering of the examples \cite{zhao2021calibrate, lu2021fantastically}. Another prompting technique that has consistently improved the output of LLMs is Chain-of-Thought Reasoning \cite{wei2022chain, chen2023you}. In this prompting scheme, the LLM is typically asked to explain its reasoning and to work through answering a prompt step-by-step. Answering prompts in such a process usually improves outcomes and helps to prevent undesirable behaviors like hallucination, where the model produces a plausible-looking answer that is incorrect \cite{wei2022chain, chen2023you}. This technique has been used in an iterative, chatting format to improve implicit sentiment classification in previous research \cite{fei2023reasoning}. Thus, while the best means of interacting with LLMs is an open research question, there are certain prompting techniques, like few-shot prompting, that can elicit better outcomes from LLMs.


